Toward 6G: From New Hardware Design to Wireless Semantic and Goal-Oriented Communication Paradigms

Several speculative visions are conjecturing on what 6G services will be able to offer at the horizon of 2030. Nevertheless, the 6G design process is at its preliminary stages. The reality today is that hardware, technologies and new materials required to effectively meet the unprecedented performance targets required for future 6G services and network operation, have not been designed, tested or even do not exist yet. Today, a solid vision on the cost-benefit trade-offs of machine learning and artificial intelligence support for 6G network and services operation optimization is missing. This includes the possible support from hardware efficiency, operation effectiveness and, the immeasurable cost due to data acquisition-transfer-processing. The contribution of this paper is three-fold. This is the first paper deriving crucial 6G key performance indicators on hardware and technology design. Second, we present a new hardware technologies design methodology conceived to enable the effective software-hardware components integration required to meet the challenging performance envisioned for future 6G networks. Third, we suggest a paradigm shift towards goal-oriented and semantic communications, in which a totally new opportunity of joint design of hardware, artificial intelligence and effective communication is offered. The proposed vision is consolidated by our recent results on hardware, technology and machine learning performance.

==> low_complexity_dpd.tex <==
\section{System model}\label{sec:sys_model}
\subsection{OFDM signal and PA impairments}\label{sec:OFDM_PA}
We consider a communication system integrating a QAM modulation, an OFDM transmitter, a DPD based on NN techniques and a PA . The communication system is shown on Figure \ref{sys_model}.
% [JB] ca n'apporte rie de savoir que c'est de la QMA ou que la taille de FFT est de 1024!
%and its parameters are described in \tabref{sys_mod_params}.

\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figure/sys_model.pdf}
    \caption{Sytem Model}
    \label{fig:sys_model}
\end{figure}

We characterize the PA with an amplitude distortion function denoted $f_{\rho}$ and a phase shift function denoted $f_{\Phi}$. The output characteristics are given by:
\begin{equation}
    |y| = f_{\rho}(|x|)
\end{equation}
\begin{equation}
   \arg(y)  =  f_{\Phi}(|x|) + \arg(x)
\end{equation}
where $x$ and $y$ are the input and output signals respectively. Assuming a PA derived from a 3GPP Rapp model for communication above 6GHz \cite{rapp3gpp}, the two functions are defined as follows:

\begin{equation}
 f_{\rho}(u) = \frac{Gu}{\left(1+|\frac{Gu}{V_{sat}}|^{2p}\right)^{\frac{1}{2p}}} \label{eq:rapp_rho}
\end{equation}
\begin{equation}
 f_{\Phi}(u) = \frac{Au^q}{\left(1+\left(\frac{u}{B}\right)^q\right)}
 \label{eq:rapp_phi}
\end{equation}
where $G$ denotes the gain in linear region, $p$ the ``knee" factor and $V_{sat}$ the saturation voltage level. $A$, $B$ and $q$ are fitting parameters.
Thereafter, we consider the following input back-off (IBO) definition :

\begin{equation}
    IBO = \frac{P_{1dB,in}}{P_{avg,in}},
\end{equation}
where $P_{1dB,in}$ corresponds to the input power at the $1dB$ compression point and $P_{avg,in}$ the average input power.

Besides, we consider our model to be noise free and interference due to non-linearities are not taken into account during training stage.

%\begin{table}[!t]
%	\centering
%	\caption{System model parameters}
%	\label{tab:sys_mod_params}
%	\renewcommand{\arraystretch}{1.25}
%	\begin{tabular}{l||c}
%	    Parameters & Values \\
%	    \hline
%	    \hline
%		Modulation          & QAM                  %    \\ \hline
%		Modulation Order    & $64$                %      \\ \hline
%		Subcarriers         & $1024$              %        \\ \hline
%		Cyclic Prefix (CP)  & $72$                %    \\ \hline
%	\end{tabular}
%\end{table}

% ------------------------------------------------------------------------------
\subsection{Conventional Neural Network DPD  (CNNDPD)}
\label{sec:low_nn}
% ------------------------------------------------------------------------------
In this section, we present our solution to perform the neural network (NN) digital predistortion (DPD) function. It is based on the indirect learning architecture (ILA), which has been shown to provide better performance compared to the direct learning one. It is worth to mention that the investigated scheme is different compared to the ones presented in the literature \cite{Zayani2007}\cite{Tarver2019}. Indeed, instead of proposing a ``blackbox" architecture, \ie some fully connected hidden layers, we decide to design our neural network to specifically tackle amplitude and phase impairments separately through a polar decomposition of the signal. According to \cite{Zayani2014}, tackling AM/AM and AM/PM distortions gives better results which motivates this choice. It results in a specific architecture.

The CNNDPD is composed of two neural networks. Each neural network represents a function correcting respectively the amplitude distortion (AM/AM) and the phase distortion (AM/PM). 

The architecture of both neural networks is presented in Figure \ref{dpd_nn_arch}. It must be emphasized that these neural networks respectively use amplitude and phase information of the signal.

\begin{figure}[htb!]%!t]
    \centering
    \subfloat[Predistorsion function for AM/AM distorsion]{
        \includegraphics[width=0.5\columnwidth]{figure/am_am_architecture}
        \label{fig:am_am_arch} 
    }
    \hfil
    \subfloat[Predistorsion function for AM/PM distorsion]{
        \includegraphics[width=0.5\columnwidth]{figure/am_pm_architecture}
        \label{fig:am_pm_arch} 
    }
    \caption{Architecture of the CNNDPD}
    \label{fig:dpd_nn_arch}
\end{figure}

\subsubsection{Neural Network for AM/AM DPD}
In this paragraph, we present the architecture of the neural network allowing to inverse the PA AM/AM characteristic represented on Figure \ref{am_am_arch}. First, it can be noticed that this architecture is fully customized in order to resolve the specific issue of inverting the PA AM/AM characteristic. Based on the system model presented in \secref{sys_model}, the NN presented here takes the output amplitude of the PA and predicts the input amplitude. This NN is optimized to find the function $\widehat{f_{\rho}^{\text{-}1}}$ such as,

% \begin{align}
%     (f_{\rho}\circ \widehat{f_{\rho}^{\text{-}1}})(|x|) &= G|x|, \\
%     \widehat{f_{\rho}^{\text{-}1}}(u) &= g_0(u) + g_1(u), \notag \\
%     g_0(u) &= \gamma_0(u) + \left(1-\gamma_0(u)\right)u, \notag \\
%     \gamma_0(u) &= \left(1+e^{-\alpha\left(u-w_0\right)}\right)^{-1}, \notag\\
%     g_1(u) &= \text{ReLu}(W_0u^T+b_0), \notag
% \end{align}

 \begin{align}
     (f_{\rho}\circ \widehat{f_{\rho}^{\text{-}1}})(|{x}|) &= G|{x}|, \\
     \widehat{f_{\rho}^{\text{-}1}}({u}) &= g_0({u}) + g_1({u}), \notag \\
     g_0({u}) &= \gamma_0({u}) + \left(1-\gamma_0({u})\right) {u}, \notag \\
     \gamma_0({u}) &= \left(1+e^{-\alpha\left({u}-\omega_\rho \right)}\right)^{-1}, \notag\\
     g_1({u}) &=  \sum_{j=1}^{N^{\rho}_n} \omega^\rho_j \left[\text{ReLu}(\mathbf{W }_\rho{u}+\mathbf{b}_\rho) \right]_j, \notag
 \end{align}
where $\alpha, \omega_\rho, \omega^\rho_j \in \mathbb{R} $, $\mathbf{W}_\rho \in \mathbb{R}^{1 \times N^{\rho}_n}$ and $\mathbf{b}_\rho \in \mathbb{R}^{1 \times N^{\rho}_n}$  are optimized during the learning phase. $N^{\rho}_n$ the number of neurons. The function $g_0$ allows to model the invert AM/AM characteristic and the function $g_1$ allows to refine the DPD function estimated by $g_0$. $\text{ReLu}$ function is defined by $f(x_i)=\max(0,x_i),  x_i = \left[ \mathbf{x}\right]_i$.

\subsubsection{Neural Network for AM/PM DPD}
We present here the NN architecture used to correct phase shift due to the PA. The NN takes the input amplitude and predict the opposite of the phase shift. The architecture is different from the NN dedicated to invert the AM/AM characteristic because here we need to find an opposite which is likely simpler. Hence, fewer operations are required resulting in lower complexity. This NN is optimized to find the function $f_{-\Phi}$ such as,

\begin{align}
    f_{\Phi}(|x|) + f_{-\Phi}(|x|) &= 0, \\
    f_{-\Phi}(u) &= \gamma_1(u) g_2(u), \notag \\
    \gamma_1(u) &= \left(1+e^{-\beta\left(u-\omega_\Phi\right)}\right)^{-1}, \notag \\
    g_2(u) &= \sum_{j=1}^{N_n^\Phi} \omega^\Phi_j\text{ReLu}\left[(\mathbf{W}_\Phi u+\mathbf{b}_\Phi)\right]_j, \notag
\end{align}
where $\beta, \omega_\Phi, \omega^\Phi_j \in \mathbb{R}$, $\mathbf{W}_\Phi \in \mathbb{R}^{1 \times N^{\Phi}_n}$ and $\mathbf{b}_\Phi \in \mathbb{R}^{1 \times N^{\Phi}_n}$ are optimized during the training phase. $N^{\Phi}_n$ the number of neurons. 
In order to acquire the phase shift $f_{\Phi}(|x|)$, we realize a simple conjugate operation,

\begin{align}
    z &= x^{*} y, \\
    z &= |x|.|y|~ e^{i(\arg(y)-\arg(x))}, \notag \\
    \arg(z) &= f_{\Phi}(|x|) , \notag
\end{align}

\subsubsection{Training}
The first approach to train our solution is by using Indirect Learning Algorithm (ILA). It consists in deriving a postdisorter and placing it before the PA to perform DPD. Learning is performed by optimizing a mean squared error (MSE) loss function using an Adam \cite{Kingma2017adam} optimizer. This training approach is known as ``conventional" because we realize a simple gradient descent to update the NN parameters. 







%% --------------------Results--------------- %%

In this paragraph, we present the performance of ``conventional" learning on static and varying PA model based on \equref{rapp_rho} and \equref{rapp_phi}. For simulation purpose, we consider that parameters of the PA model are fixed according to \cite{rapp3gpp}, \ie $p=1.1$, $V_{sat}=1.9V$, $G=16$, $A=-345$, $B=0.17$ and $q=4$. The PA characteristics, AM/AM and AM/PM distorsions are presented on Figure \ref{pa_char}.

Figure \ref{evm_ila} presents the Error Vector Magnitude (EVM) in function of the Input Back-Off (IBO) using a PA which presents AM/AM and AM/PM distorsions. The ``Limit" curve corresponds to a PA linear until its saturation characterized by $\min(G|x|, V_{sat})$. The performance of our solution is almost optimal using only $10$ neurons which justify the low-complexity aspect. It must be emphasized that such a solution requires a large amount of data for a single state of our PA, about $10^5$ OFDM symbols which represents a cumbersome database. The parameters of the CNNDPD are given in \tabref{cnndpd_params}.

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figure/pa_characteristic.pdf}
    \caption{AM/AM and AM/PM characteristics of Rapp PA [8]}
    \label{fig:pa_char}
\end{figure}


\begin{table}[!t]
	\centering
	\caption{Implementation parameters of CNNDPD}
	\label{tab:cnndpd_params}
	\renewcommand{\arraystretch}{1.25}
	\begin{tabular}{l||c}
	    Parameters & Values \\
	    \hline
	    \hline
		$N_n^\rho$               & $8$                      \\ \hline
		$N_n^\phi$               & $4$                       \\ \hline
		Batch size          & $128$                      \\ \hline
		Total data          & $10^5$                    \\ \hline
		Epochs              & $50$                      \\ \hline
		Optimizer           & {Adam}                    \\ \hline
		Learning rate       & {0.001}                   \\ \hline
		Loss function       & {Mean Squared Error}    \\ \hline
		Activation function & {ReLu}                    \\ \hline
	\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figure/ila_perf_64qam_ibo3_am_pm.pdf}
    \caption{EVM performance in [dB] using ``conventional" learning}
    \label{fig:evm_ila}
\end{figure}
